FasterRisk: Fast and Accurate Interpretable Risk Scores

Over the last century, risk scores have been the most popular form of predictive model used in healthcare and criminal justice. Risk scores are sparse linear models with integer coefficients; often these models can be memorized or placed on an index card. Typically, risk scores have been created either without data or by rounding logistic regression coefficients, but these methods do not reliably produce high-quality risk scores. Recent work used mathematical programming, which is computationally slow. We introduce an approach for efficiently producing a collection of high-quality risk scores learned from data. Specifically, our approach produces a pool of almost-optimal sparse continuous solutions, each with a different support set, using a beam-search algorithm. Each of these continuous solutions is transformed into a separate risk score through a "star ray" search, where a range of multipliers are considered before rounding the coefficients sequentially to maintain low logistic loss. Our algorithm returns all of these high-quality risk scores for the user to consider. This method completes within minutes and can be valuable in a broad variety of applications.

==> sections/06-checklist.tex <==
\newpage
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{See the Limitations section in Appendix~\ref{app:discussion_of_limitation}.}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerYes{See the Limitations section in Appendix~\ref{app:discussion_of_limitation}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{app:theoretical_upper_bound_derivation}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{}
    \answerYes{The code and README are included as part of the supplemental material. Data links are included in the Appendix~\ref{app:dataset_information}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    % \answerTODO{}
    \answerYes{We perform 5-fold CV as specified in Section \ref{sec:experiments}. Hyperparameters are already specified (default values) in Algorithm \ref{alg:overall_algorithm} of Section \ref{sec:methodology}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    % \answerTODO{}
    \answerYes{See Section \ref{subsec:experiments_solution_quality}. Error bars are included for the 5-fold CV.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \answerYes{See Appendix \ref{app:computing_platform}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerTODO{}
    \answerYes{See Appendix \ref{app:baseline_specifications} and the References}
  \item Did you mention the license of the assets?
    % \answerTODO{}
    \answerYes{See Appendix \ref{app:baseline_specifications}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    % \answerTODO{}
    \answerYes{Our code is included as part of the supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    % \answerTODO{}
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\end{enumerate}
